Joint Demosaicking / Rectification of Fisheye Camera Images using Multi-color Graph Laplacian Regularization

To compose a 360 image from a rig with multiple fisheye cameras, a conventional processing pipeline first performs demosaicking on each fisheye camera's Bayer-patterned grid, then translates demosaicked pixels from the camera grid to a rectified image grid---thus performing two image interpolation steps in sequence. Hence interpolation errors can accumulate, and acquisition noise in the captured pixels can pollute neighbors in two consecutive processing stages. In this paper, we propose a joint processing framework that performs demosaicking and grid-to-grid mapping simultaneously---thus limiting noise pollution to one interpolation. Specifically, we first obtain a reverse mapping function from a regular on-grid location in the rectified image to an irregular off-grid location in the camera's Bayer-patterned image. For each pair of adjacent pixels in the rectified grid, we estimate its gradient using the pair's neighboring pixel gradients in three colors in the Bayer-patterned grid. We construct a similarity graph based on the estimated gradients, and interpolate pixels in the rectified grid directly via graph Laplacian regularization (GLR). Experiments show that our joint method outperforms several competing local methods that execute demosaicking and rectification in sequence, by up to 0.52 dB in PSNR and 0.086 in SSIM on the publicly available dataset, and by up to 5.53dB in PSNR and 0.411 in SSIM on the in-house constructed dataset.

==> conclude.tex <==
%Fisheye cameras has been of great interest for virtual reality and augmented reality applications in recent decades. 
%Direct demosaicking of a raw fisheye camera image, \textit{i.e.}, a Bayer-patterned image, would always propagate the acquisition noise of each of the three color channels to other pixel locations.  
%Inspired by state-of-the-art joint demosaicking / denoising (JDD) methods that aim to alleviate the above problem,
\vspace{-0.05in}
To alleviate the noise-propagation problem caused by conventional separate demosaicking and rectification processes on the Bayer-patterned image captured by a fisheye camera,
in this paper, we propose the first joint demosaicking / rectification framework that demosaick the Bayer-pattern and remove the fisheye camera distortion, simultaneously.
%This is opposed to the JDD methods that conduct the demosaicking and rectification processes, separately.
We do this by first interpreting the gradients of different color pairs on a Bayer-patterned image patch as noisy observations of the ones of target image patch,
and then formulating a \textit{maximum likelihood estimate}(MLE) problem.
We solve it by constructing a combinatorial graph that reflects the inter-pixel gradients of the target image patch.
Experimental results on two fisheye camera image datasets confirm that our joint demosaicking / rectification method outperforms the competing methods that demosaick and rectify the fisheye camera images, separately.

==> overview.tex <==
\begin{figure}[htb]
	\centering
	\includegraphics[width=8cm]{fig/workflow.pdf}
	\vspace{-0.10in}
	\caption{System workflow.}
	\label{fig:workflow}
\end{figure}

As shown in Fig.\,\ref{fig:workflow}, given an image patch $\x$ in the final demosaicked, rectified image, 
we first compute a mapping matrix $\H$ given the intrinsic and extrinsic parameters of the fisheye camera; 
$\H$ maps the pixels between the Bayer-patterned image and the demosaiced, rectified image. 
We then construct an 8-connected graph for each of the red, green, and blue channels of the demosaiced, recitified image,
which in turn defines a graph Laplacian $\L$.
We next iteratively update $\x$ and $\L$ based on our joint demosaicing / rectification formulation until convergence.




==> related.tex <==
\vspace{-0.05in}
There are recent efforts to address inverse imaging problems using graph spectral techniques, including image denoising \cite{7814302}, soft decoding of JPEG images \cite{7740964}, image deblurring \cite{8488519} and join dequantization / contrast enhancement \cite{8476571}.
Though the details of the employed graph-based regularizers differ across applications, the key to good reconstructed image quality remains the same: to appropriately design an underlying graph that captures inter-pixel similarities of the target image patch. 
Our current work differs from these works in that we estimate the gradient (difference) of a target color pixel pair in the rectified image grid using relevant observed gradients in the Bayer-patterned grid in all three color components. 

In the computer vision literature, there have been numerous recent attempts to jointly demosaick and denoise a Bayer-patterned image \cite{1658081,4287011,Gharbi:2016:DJD:2980179.2982399,DBLP:journals/corr/abs-1802-04723}.
%Specifically, \cite{1658081} adopts a total least squares method to simplify the JDD problem as a single-color denoising problem. \cite{4287011} first recovers the green channel by exploiting both spectral and spatial correlations among three channels, and use that result to guide the recovery of the other two channels. Both \cite{Gharbi:2016:DJD:2980179.2982399} and \cite{DBLP:journals/corr/abs-1802-04723} adopt data-driven approaches to optimize the reconstruction quality. Inspired by these efforts, our proposal is to jointly perform demosaicking and rectification from a fisheye-camera-captured image. Though one can alternatively demosaick the Bayer-patterned image and rectify it to the target 2D image grid separately, performing the two tasks jointly means that additive noise experienced at the image sensor is addressed directly at the final rectified image grid, where piecewise smooth (PWS) reconstruction (promoted using GLR) is known to be desirable for objective and subjective image quality. 
%\textit{ To the best of our knowledge, we are the first to perform joint demosaicking / rectification for fisheye-camera-captured images in the literature. }
